AdaSplit: Adaptive Trade-offs for Resource-constrained Distributed Deep Learning

Distributed deep learning frameworks like federated learning (FL) and its variants are enabling personalized experiences across a wide range of web clients and mobile/IoT devices. However, FL-based frameworks are constrained by computational resources at clients due to the exploding growth of model parameters (eg. billion parameter model). Split learning (SL), a recent framework, reduces client compute load by splitting the model training between client and server. This flexibility is extremely useful for low-compute setups but is often achieved at cost of increase in bandwidth consumption and may result in sub-optimal convergence, especially when client data is heterogeneous. In this work, we introduce AdaSplit which enables efficiently scaling SL to low resource scenarios by reducing bandwidth consumption and improving performance across heterogeneous clients. To capture and benchmark this multi-dimensional nature of distributed deep learning, we also introduce C3-Score, a metric to evaluate performance under resource budgets. We validate the effectiveness of AdaSplit under limited resources through extensive experimental comparison with strong federated and split learning baselines. We also present a sensitivity analysis of key design choices in AdaSplit which validates the ability of AdaSplit to provide adaptive trade-offs across variable resource budgets.

==> content_new/ablations.tex <==
\section{Discussion}
\ref{sec:ablations}
From the results, we observe that SL++ provides two key benefits, over baselines,: i) improved performance under limited resources, ii) ability to adapt to variable resource budgets. Section ~\ref{sec:results} focused on the former, we delineate the latter here. To do so, we conduct sensitivity analysis of key design choices that make SL++ flexible. Unless specified otherwise, hyperparameters are $\kappa=0.6$, $\eta=0.6$.

% computation
\subsection{Size of Client Model}
Since the server model is only trained intermittently, it is natural to question how size of client model impacts trade-off. Table ~\ref{tab:client-size-cifar} presents results by varying number of layers of client with \textif{Mixed-CIFAR10} dataset. Trivially, client \textbf{computation} cost scales monotonically with increase in client layers. Interestingly, we also observe a decrease in bandwidth with increase in client size. This can be attributed to our convolutional architecture where size of activation maps decrease along depth and results in reduced payload. Importantly, we note that accuracy is largely insensitive to size of client size. We note slightly better convergence with larger server model since it provides more parameters to regulate collaboration. We observe similar trends on \textit{Mixed-NonIID} and results are presented in Appendix.

% computation and communication
\subsection{Interrupt Duration}
Table ~\ref{tab:interrupt-duration} presents results on \textit{Mixed-CIFAR10}. Increasing $\kappa$ directly decreases communication and computation cost. Communication decreases as $P_{is} = 0$ for duration of all rounds $r < \kappa$. This is corroborated with a decrease in bandwidth consumed. While client compute is unchanged, server computation decreases significantly. We note marginal decrease in accuracy since higher $\kappa$ allows for fewer collaboration iterations on server. Specifically, as $\kappa$ increases from 0.3 to 0.9, bandwidth falls from 17.22 GB to 2.43 GB. Correspondingly, accuracy decreases from 89.80\% to  87.11\%. This can provide adaptive trade-off to SL++.

% computation and communication
\subsection{Eliminating Gradient Flow}
In SL++, client does not receive gradient from the server. Table ~\ref{tab:gradient-flow} analyses the impact of this choice on \textit{Mixed-CIFAR10}. We observe direct implication on communication cost with bandwidth reduced by one-half (as size of total payload decreases). We observe that accuracy does not decrease though there is slight increase in the standard deviation. Results on \textit{Mixed-NonIID} corroborate observation and are included in the appendix.

% communication
\subsection{Activation Sparsity}
Strategies in SL++ for each dimension are not exhaustive. Here, we consider sparsification of the split activations. During training, an $L^{1}$ is added to client loss constrain magnitude of activations. Results are presented on \textit{Mixed-NonIID} in Table  ~\ref{activation-sparsity}. \textit{Computation} remains unchanged. \textit{Communication} decreases as payload ($P_{ij}$) becomes sparse. This results in fall in accuracy which highlights worsening collaboration. Specifically, we observe that performance decreases to 76\% as bandwidth falls to 0.48 GB. However, we note that this can enable SL++ to support extremely low-bandwidth setups.

% collaboration
\subsection{Client Attention}
SL++ improves collaboration between heterogenous clients by learning multiplicative masks when updating shared weights. Here, we consider an alternate strategy. In addition to the multiplicative mask, we also learn client specific additive parameters which are weighted by inter-client attention. Correspondingly, the weights each client can update are represented as:
\begin{equation}
    \theta_c = \theta_{shared} \odot m_c + a_c + \sum_{i \ne c} \alpha_{ci} a_{i}
\end{equation}

For each client, server parameters are trained with the following objective.
\begin{equation}
    \min_{m_c, a_c, \alpha_{c,:} \theta_{shared}} L_{ce} + \lambda \Omega (\{m_c, a_c\})
\end{equation}

Results are reported on \textbf{Mixed-NonIID} in Table ~\ref{tab:client-attn}. We observe improved collaboration but at cost of increase in computation. Communication cost is unchanged. We visualize the inter-client attention mask in Figure ~\ref{fig:attn-mask} which shows higher activations for clients with more similar data, validating effectiveness of technique. Importantly, this validates adaptability of SL++ to improve collaboration under higher computation budgets.

==> content_new/method_backup.tex <==
% motivation, key insight, algorithm, trade-off

\section{AdaSplit}
\label{ref:method}
In this section, we delineate the design choices of AdaSplit along each of the three dimensions. We also discuss corresponding trade-offs that enable AdaSplit to adapt to variable resource constraints. Unless specified otherwise, we follow the same notation as defined in Section ~\ref{sec:prelim}.

\subsection{Computation}
\label{ref:slpp-compute}
% specific design
The training model is split between the client and server. Following split learning, each client is characterized by a local client model $M^{c}_{i}$ and global server model $M^{s}$ that is shared across all clients. This flexibility to distribute model allows scaling SL (and AdaSplit) to low resource setups. However, in SL, this increases computation load on server and also blocks the server to train synchronously with each client model which depends upon the server for gradient.

AdaSplit alleviates these concerns by eliminating dependence of the client model on server gradient and only training the server intermittently. This further lowers the total computation cost by decreasing $T_{s}$ (compute iterations on server) and also unblocks the server to execute asynchronously from the client. 

% generate local gradient + send activations sporadically to server.
\textbf{Local Client Gradient:} \textit{First}, AdaSplit generates the gradient for training client model using a local objective function $L_{client}$ which is a supervised version of NT-Xent Loss \cite{NIPS2016_6b180037}. Given an input $(x_{i}, y_{i} \sim D_{i})$, $L_{client}$ is applied on a projection of the activations $a_{i}$ generated using the client model ($=M^{c}_{i}(x_{i})$). The projector $H(.)$ is used to produce a 64-dim vector on which the loss is applied. Let $q_i = H(a_i)$ be an embedding of an input $x_i$, and $Q^{i}_{+}$ be the set of embeddings of other inputs with the same class as $x_i$ in the batch with batch-size $b$, the loss can be represented as below:

\begin{equation}
    L_{client} = \sum^{b}_{i=0} \sum_{q_{+} \in Q^{i}_{+}} -\log \frac{exp(q_i \cdot q_{+}/\tau)}{\sum^{b}_{j \ne i} \cdot exp(q_i \cdot q_j/\tau)}
\end{equation}

Here, $\tau$ is a hyperparameter, which controls the "margin" of closeness between embeddings. We set $\tau = 0.07$ in all our experiments.
The pairs (anchor, positive inputs) required in $L_{client}$ are sampled using the ground truth labels ($y_{i}$) present locally on the client device.

\textbf{Intermittent Server Training:}\textit{Second}, AdaSplit also \textit{splits} the $R$ round training into two phases: A) INTERRUPT PHASE B) POST-INTERRUPT PHASE. Interrupt Phase lasts for the first $K$ rounds when only the client model trains, asynchronously and without interacting with the server, using $L_{client}$. After $K$ rounds, the client starts interacting with the server by transmitting activations. Only now the server model starts training on data from the given client. The server model $M^{s}$ is optimized using a server loss function ($L_{server}$) which is the cross entropy objective for classification experiments. We note that the client model continues to train $L_{client}$ and does not receive any gradient from the server. 

Essentially in AdaSplit, local client model leverages compute resources of server only when required. AdaSplit can adapt to variable computation budgets by regulating two key hyperparameters: i) size of the client model, ii) duration of interrupt phase. We study the specific impact of these design choices in Section ~\ref{sec:ablations}. Also, in practice, we observe considerable reductions in total computation since $K$ can assume large values (0.8*R) without significant loss of performance. We corroborate this with experiments in Section ~\ref{sec:results}.

% We observe that for local training, using the contrastive loss is a better alternate than cross entropy objective. This is because $L_{con}$ not only improves performance but also prevents large increase in client computation required to by the parameters to project (flattened) activations to the label space. This also enables scaling local client model training even when label space is large.

\subsection{Communication}
\label{ref:slpp-comm}
In split learning, the high frequency of client-server interaction can be prohibitive for communication cost. AdaSplit reduces this by decreasing payload size as well as the frequency of communication. The key idea is to only have \textit{subset} of clients interact \textit{intermittently} with the server.

\textbf{Smaller Payload:} \textit{First}, we note that eliminating client dependence on server gradient also significantly reduces communication bandwidth, apart from decreasing computation. In AdaSplit, for each client $i$, $P_{si} = 0$ throughout training. Furthermore, during interrupt phase, also $P_{is} = 0$ since only client model trains locally and no activations are communicated to server.

\textbf{Infrequent Transmission:} \textit{Second}, in the post-interrupt phase, only subset of clients communicate activations to the server to train the server model $M^{s}$ in each round. This manifests as an orchestrator on the server which executes a multi-arm bandit strategy to selects a subset for each round. The intuitive goal is to trade-off prioritizing clients which require access to server model to improve performance (exploitation) while also ensuring that the final model can generalize when to the different client data distributions (exploration). Specifically, at each batch, a subset of $K$ ($< N$) clients is selected as follows: At iteration $t$, i) Selected clients (i.e. $S^t_c = 1$) are trained on a batch of their training data, then loss $L^{t}_{c}$ of each client $c$ is stored. ii) For clients which weren't selected (i.e. $S^t_c = 0$), we estimate their loss as the average of previous two iterations i.e. $L^{t}_{c} = \frac{L^{t-1}_{c} + L^{t-2}_{c}}{2}$ iii) Server orchestrator assigns a score to each client using an exponential sum of running $L^{t}_{c}$ history using the advantage function. This score is normalized by prior selection count of the client to boost exploration. iv) Clients with top-K scores are selected for server communication. The advantage function is defined below:
\begin{equation}
    l_c = \sum^{T}_{t=0}\gamma^{T-1-t} \cdot L^{t}_{c}
\end{equation}
\begin{equation}
    s_c = \sum^{T}_{t=0}\gamma^{T-1-t} \cdot S^{t}_{c}
\end{equation}
\begin{equation}
    A_c = \frac{l_c}{s_c} + \sqrt{\frac{2 \log T}{s_c}}
\end{equation}
$\gamma \in [0, 1]$ is a hyperparameter that determines the importance of historical values. If $\gamma = 1$, then older values are weighed to be as important as the most recent value; if $\gamma = 0$, then historical values are completely ignored and only the most recent value is used for computing the advantage function. We initialize $L^{t}_c = 100$ for all clients for $t=0$ and $t=1$.

AdaSplit can adapt to variable communication budgets by regulating two key hyperparameters: i) number of selected clients, ii) duration of interrupt phase. We study the specific impact of these design choices in Section ~\ref{sec:ablations}. In practice, we observe considerable reductions in communication cost since $K$ (0.8*R) and $S$ (0.6*S) can assume large values without significant loss of performance. We corroborate this with results in Section ~\ref{sec:results}.

\subsection{Collaboration}
\label{ref:slpp-collab}

The key idea is to regulate interference by constraining each client to update only a subset of model parameters. The motivating insight is to take advantage of the fact that neural networks are vastly over-parameterized and only a small subset of the parameters are needed to successfully learn each client's task. For reducing interference, when a client $c$ is communicating with the server, it only updates it's own parameters, i.e. the multiplicative mask $m_c$ and the shared parameters $\theta_{shared}$. For each client, the final weights $\theta_c$ is computed as:
\begin{equation}
    \theta_c = \theta_{shared} \odot m_c
\end{equation}

Here, we force $m_c$ to be extremely sparse using $L^1$ regularization, i.e. $\Omega(.)$. Each client $c$, when communicating with the server, optimizes the following objective:
\begin{equation}
    \min_{m_c, \theta_{shared}} L_{ce} + \lambda \Omega (m_c)
\end{equation}
Here, $\lambda$ is a hyperparameter that controls sparsity of the masks, in other words, $\lambda$ controls the degree of collaboration between clients.


==> content_new/results.tex <==
\section{Results}
\label{sec:results}
We report performance for ~\textbf{Mixed-CIFAR} in Table ~\ref{tab:split-cifar} and  ~\textbf{Mixed-NonIID} in Table ~\ref{tab:non-iid}. The results, in both settings, present two key observations: i) SL++ consistently outperforms both split and federated learning baselines under limited resources, ii) SL++ can adapt to variable resource budgets. 


\textbf{Mixed-CIFAR: } Results are summarized in Table ~\ref{tab:split-cifar}. For computing \textbf{C3-Score}, we set $B_{max} = 35.94 GB$ and $C_{max} = 11.77 TLOPS$, which are the highest bandwidth and computation cost for any method. \textit{First,} \textbf{SL++} consistently provides the \textbf{best trade-off among all} of federated and split learning baselines. Specifically, SL++ achieves a \textit{C3-Score} of 0.89 with the closest federated learning baseline (FedProx) at 0.81, FedAvg at 0.79 while SplitFed is at 0.62. \textit{Second,} SL++ achieves significantly better accuracy that both other split learning  techniques while also reducing bandwidth consumption. Specifically, in comparison to vanilla SL, SL++ \textbf{improves performance by 24\%} and consumes \textbf{89\% lower} bandwidth. \textit{Third,} SL++ makes split learning a competitive alternate to federated learning. We observe SL++ achieves consistently higher (or similar) accuracy that federated learning baselines with significantly lower client compute and similar bandwidth. Specifically, SL++ 91.92\% accuracy while consuming 2.85 GB bandwidth and 2.38 TFLOPS client compute. This is 3\% higher than FedNova which also consumes 6 times more compute and similar bandwidth. FedProx achieves similar performance (92.54) but consumes 6 times the bandwidth. This is also corroborated through C3-Scores (0.89 for SL++ vs 0.81 for FedProx, 0.77 for FedNova).
\textbf{Fourth,} SL++ can adapt to variable resource budgets. Given a higher bandwidth budget, we see that SL++ can further improve accuracy to 93.02\%. This tunability of SL++ is immensely powerful in real-world setups and we observe it is captured by the C3-Score.


\textbf{Mixed-NonIID: } Results are summarized in Table ~\ref{tab:non-iid}. For computing C3-Scores, we set $B_{max} = 84.54 GB$ and $C_{max} = 17.13$ which are the highest bandwidth and computation cost for any method (Vanilla SL and FedProx respectively). \textit{First,} SL++ consistently provides the \textbf{best trade-off among all} of federated and split learning baselines. Specifically, SL++ achieves 
